Silhouette: Efficient Protected Shadow Stacks for Embedded Systems

Microcontroller-based embedded systems are increasingly used for applications that can have serious and immediate consequences if compromised---including automobile control systems, smart locks, drones, and implantable medical devices. Due to resource and execution-time constraints, C is the primary language used for programming these devices. Unfortunately, C is neither type-safe nor memory-safe, and control-flow hijacking remains a prevalent threat. This paper presents Silhouette: a compiler-based defense that efficiently guarantees the integrity of return addresses, significantly reducing the attack surface for control-flow hijacking. Silhouette combines an incorruptible shadow stack for return addresses with checks on forward control flow and memory protection to ensure that all functions return to the correct dynamic caller. To protect its shadow stack, Silhouette uses store hardening, an efficient intra-address space isolation technique targeting various ARM architectures that leverages special store instructions found on ARM processors. We implemented Silhouette for the ARMv7-M architecture, but our techniques are applicable to other common embedded ARM architectures. Our evaluation shows that Silhouette incurs a geometric mean of 1.3% and 3.4% performance overhead on two benchmark suites. Furthermore, we prototyped Silhouette-Invert, an alternative implementation of Silhouette, which incurs just 0.3% and 1.9% performance overhead, at the cost of a minor hardware change.

==> codesize.tex <==
%------------------------------------------------------------------------------%
\subsection{Code Size Overhead Analysis}
\label{section:results:mem}
%------------------------------------------------------------------------------%
%
% experiments to run:
% - memory overhead of baseline programs v.s. transformed programs
% - memory overhead of each instrumented instruction (put in appendix).
%

\input{tables/code_size}

Low code size overhead is important for embedded systems as they usually have
limited memory.
We measured the code size overhead incurred by {\System} by measuring
the code size of the BEEBS benchmarks, the code in the HAL
library that is compiled and linked into the benchmark executable, 
the MPU configuration file, and the benchmark's {\tt main()} function. 
As Section~\ref{section:impl:limitation} mentions, {\System} currently does
not instrument the startup files or the C standard library, so our
measurements do not include sizes of their functions.
Table~\ref{table:codesize} shows the code size measurement results.

\paragraph{Shadow Stack Code Size}
The shadow stack instrumentation adds a small amount of overhead.
The arithmetic mean is 2.55\%, and the highest overhead is only 3.76\%.  Our
shadow stack implementation adds additional instructions in a function's
prologue and epilogue,
as Section~\ref{section:impl:ss} describes. Therefore, it incurs higher overhead 
on programs that contain more none-leaf functions, i.e., functions that push the
return address onto the stack. For programs that have functions with 
multiple epilogues (functions that can return from multiple sites), their code 
size overhead is usually higher than average as well.
Some programs, such as \emph{tarai} and \emph{recursion}, show
high overhead, but the increase of actual code
size is not significant compared to other benchmark programs because
these programs are relatively small and most of the overhead comes
from the {\tt main()} function and functions in the HAL library.  

\paragraph{CFI Code Size}
The CFI transformation induces negligible overhead.
The highest overhead is 5.64\% from {\tt picojpeg}, which contains 
a large number of indirect branches. All other programs
show overheads less than 2\%. The arithmetic mean is only 1.20\%.
As mentioned in Section~\ref{section:results:perf}, most BEEBS programs
do not make heavy use of indirect branches. Therefore, the CFI pass 
does not add many new instructions to most of the BEEBS programs.

\paragraph{Store Promotion Code Size}
Store promotion incurs the most space overhead of {\System}.  
By arithmetic mean, store promotion incurs 12.75\% of overhead.  The highest
overhead is 19.53\% from {\tt ndes}. 
As discussed in Section~\ref{section:impl:store} and shown in
Table~\ref{table:store}, {\ISA} has many variations of regular store 
instructions but only supports three unprivileged stores.
Therefore, {\System} transforms some regular store instructions
into a sequence of multiple instructions. 
The most problematic store instructions are floating-point stores and
stores that write multiple registers to contiguous memory locations.
Transforming a store of a single-precision floating-point register
generates at least 4 new instructions, incurring at least 10~bytes of overhead.
To store a double-precision floating point register, as Listing~\ref{fig:vstr}
shows, the code size overhead would be no less than 20~bytes.
A Store Multiple ({\tt STM})~\cite{ARMv7M} instruction can store up to 13
general purpose registers,  and a Floating-point Store Multiple
instruction ({\tt VSTM})~\cite{ARMv7M} can store up to 16 double-precision
(64-bit) registers to memory.  We have seen
cases in which store promotion transforms a 4-byte {\tt VSTM}
instruction to a set of unprivileged store instructions inducing
more than 100 bytes of overhead.  Table~\ref{table:codesize} shows that 
programs that use more floating-point operations, such as {\tt select} and
{\tt nbody}, usually incur high code size overhead.

\paragraph{Full {\System} Code Size}
With all the three passes turned on, {\System} incurs an arithmetic mean of 
16.93\% code size overhead.  The highest overhead is 23.41\%
and the lowest is 10.57\%.

\paragraph{{\SystemInvert} Code Size}
{\SystemInvert} incurs an arithmetic mean of 5.40\% code size overhead.  The
highest overhead is 7.67\%, and the lowest is 1.73\%. Similar to performance
overhead, {\SystemInvert} incurs significantly lower average code size overhead
comparing to {\System} because {\SystemInvert} does not run Store Promotion
pass, which incurs the highest code size overhead. 

% In addition to performance overhead, We measured the
% code size overhead incurred by {\System}. There are no dynamic libraries,
% and both the application and library code are linked into one binary
% executable file. We measured the code size of the functions of BEEBS programs
% and the HAL library; we only count those functions that are both compiled by
% {\System} and linked into the binary.  Although the code size measured by
% {\System} is not exactly the same as the binary (as mentioned
% Section~\ref{section:impl:limitation}, currently {\System} does not instrument
% libcrt runtime library and C standard library), we believe that our
% measurements accurately show the space impact brought by {\System}.  We use
% the {\tt getInstrSizeInBytes()} method from the {\tt ARMBaseInstrInfo} class of
% LLVM to compute the size of each machine instruction. Table~\ref{table:codesize}
% shows the results.

% The highest overhead is only 22.95\% and
% the lowest is 8.96\%. The arithmetic mean is 15.05\%. There are two kinds of
% stores instructions that would cause high code size overhead when transformed.
% One is floating-point store. As discussed in Section~\ref{section:impl:store},
% transforming a store of a single-precision register would generate at least 5
% new instructions, incurring at least a 10-byte overhead.  To store a
% double-precision register, the code size overhead would be no less than 16
% bytes. The other kind is Store Multiple stores. An {\tt STM} can store up to 13
% general purpose registers. The situation gets even worse when Floating-point
% Store Multiple store happens: a {\tt VSTM} can store up to 16 double-precision
% (64-bit) registers to consecutive memory locations. Sometimes a 4-byte {\tt
% VSTM} can grow to more than 100 bytes.  Table~\ref{table:codesize} shows that 
% programs with intensive floating-point operations, such as {\tt minver} and {\tt
% nbody}, usually incur high code size overhead.

% \Comment{JZ: If we have time, it's nice to figure out how much overhead is from
% the transformation of floating-point registers and how much is from integer
% registers.}





==> future.tex <==
%==============================================================================%
\section{Future Work}
\label{section:future}
%==============================================================================%


% We have the following future work to do. First, we will finish implementing the
% shadow stack and the CFI. Second, we will investigate CFI techniques to find or
% design a solution more precise and more suitable for real-time embedded systems.
% Third, we will examine the inline assembly code in the test programs, and
% transform the C standard library and runtime library to make {\System} more
% complete. Lastly, we will test more programs.
% \Comment{JZ: Rewrite the future work paragraph after we finish all the
% implementation and experiments.}


%
% Outline:
%
% o Improvements to {\System}: better call graph
% o Using isolation on embedded OS components: saved program state
% o Architecture improvements to store instructions on ARM
%

We see three primary directions for future work.
First, we can optimize {\System}'s performance.
For example, Section~\ref{section:security:ss_integrity} shows that
{\System} ensures that the stack pointer stays within the stack region.
Consequently, store instructions using {\tt SP} and an immediate to
compute target addresses are unexploitable;
{\System} could elide {\storetechnique} on such stores.
Second, we can reduce the annotation effort for the HAL library by
employing privilege overlaying from EPOXY~\cite{EPOXY:Oakland17}
to identify HAL functions that should not be transformed by {\storetechnique}.
\Comment{JZ: I think the second item may confuse readers. We only briefly
mention in the threat model section that HAL is ``either compiled separately
from the application code or is annotated''. It's highly possible readers
have forgotten that and felt confused with why we talk about annotation
effort for the HAL when they read this section.}
Third, we can use {\System} to protect other memory
structures, such as the safe region used in CPI~\cite{CPI:OSDI14} and
the process state saved on interrupts and
context switches (like previous work~\cite{KCoFI:Oakland14} does).


==> survey.tex <==
%==============================================================================%
\section{Control Flow Hijacking Defenses}
\label{section:survey}
%==============================================================================%
%
% - explain what is forward and what is backward control flow transfers.
% - 

\Comment{JZ: Since this is not a survey paper, there's no need to use a whole
section to discuss existed defenses. We can briefly talk about CFI and 
incorporate the shadow stack stuffs into the Design section.}

A survey paper~\cite{CFISurvey:CSUR17} classifies the control flow of a program
into two types: forward and backward. A forward transfer of control flow
branches to a new place in the program. The most common forward transfers are
function calls, directly or indirectly via function pointers. Broadly speaking,
backward control flow can be any transfers branching to a previous memory
location, such as from the end to the beginning of a loop. In this work, we
restrict backward control flow to be only returning from a callee to its caller;
and for forward control flow transfer, we focus on protecting indirect function
calls.

In this section, we discuss two major categories of defense policies that
protect the control flow of a program. We discuss Control-Flow Integrity (CFI)
for protecting the forward transfers of control flow and Shadow Stack for
protecting the backward transfers of control flow. We focus on these two
defenses because {\System} they are relatively efficient and effective among all
the state-of-the-art control-flow protection techniques.

%------------------------------------------------------------------------------%
\subsection{Control-Flow Integrity}
\label{section:survey:CFI}
%------------------------------------------------------------------------------%
%
% - Why do we need CFI?
% - What limitations does CFI have?
% - Why cannot CFI handle backward transfers well?
%

The core of any code-reuse attack is to hijack the control flow of a program and
redirect them to the predetermined memory locations chosen by an attacker.
Since the destinations of direct control flow transfers (conditional branches
and direct function calls) are determined during compilation time and are
usually hard-coded into the native code, it is almost impossible to modify them
on a system with the ``write or execute'' protection turned on.  Thus, indirect
control flow transfers, mainly indirect function calls and returns from function
calls, are of great interest to attackers. Starting from a simply memory safety
error such as buffer overflow, a smart and sophisticated attack can hijack the
control flow of the program by rewriting the target destinations of indirect
transfers. 

The fundamental idea of Control-Flow Integrity (CFI)~\cite{CFI:CCS05} is
restricting the possible destinations of any indirect branch. A CFI policy
consists of two components: a Control-Flow Graph (CFG) representing the legal
control flow transfers of the program and a dynamic checking mechanism to check
the validity of all control flow transfers according to the CFG when the program
is running. A CFI policy usually puts labels at destinations of all possible
indirect branches, and instruments each indirect branch instruction with
instructions to be executed during runtime to determine if the control flow
transfer is legit by checking the expected labels. The efficacy of a CFI policy
is mainly determined by the precision of the CFG. However, a predetermined CFG
prior to runtime is always over-approximated for soundness. To date, most CFI
policies focus on generating and using a static CFG during compilation
time~\cite{CFI:CCS05,CFISandboxing:CCS11,CFICompiler:SEC14,KCoFI:Oakland14}.  To
improve precision, CFI policies utilizing dynamic CFG have also been studied and
proposed~\cite{CFIPerInput:CCS15,UCTCFI:CCS18}. 

The security guarantees of a CFI-enforced program also depend on how the
validity of the transfers is checked during runtime. The precision of the CFG
determines how secure a CFI policy can be, and the dynamic checking determines
how secure a program will actually be. Ideally, an indirect control flow
transfer should only branch to destinations allowed by the CFG, but this
enforcement is often too expensive in practice. However, Abadi et al. argued
that even coarse-grained CFI can bring significant security
improvement~\cite{CFI:CCS05}.  For example, in an extreme case, a whole program
only has two labels: one is inserted at the beginning of each function and one
is inserted after each indirect function call instruction. This two-label CFI
guarantees that an indirect function call can only branch to the beginning of a
function, and a return instruction can only return to the instruction after a
function call.  Although this design still opens space for control-flow
hijacking attacks~\cite{OutOfControl:Oakland14}, it already considerably
decreases the number of code gadgets available for an attacker to exploit and
largely increases the difficulty of exploitation.

%------------------------------------------------------------------------------%
\subsection{Shadow Stack}
\label{section:survey:shadow}
%------------------------------------------------------------------------------%
%
% - would TOCTOU be a problem?
% - would setjmp/longjmp be a problem?
%
% First, describe how a typical shadow stack works.
% Second, describe a few different shadow stacks.
%

Return-Oriented Programming (ROP)~\cite{ROP:CCS07,ROP:TISSEC12,ROP:USS14} is one
of the most powerful and popular attacks to exploit the corruption of return
addresses. One
key step of ROP is to find and corrupt desired return addresses of function
calls, without which ROP cannot succeed. Naturally we would like to keep the
return addresses incorruptible. However, this is very difficult on modern ISAs
like x86 and ARM: the call chain of a program can be arbitrarily long, and thus
return addresses have to be stored on the stack, which requires to be writable.
For programs written in a memory-unsafe language like C, it is extremely
challenging to differentiate between the legit and the malicious writes to the 
stack.

Shadow stack~\cite{RAD:ICDCS01,SS:AsiaCCS15,SSSok:Oakland19} is a mechanism to
keep the integrity of return addresses by maintaining a separate stack dedicated
to preserve all the live return addresses on the regular stack. When it comes to
use a return address, the program either checks if the return address matches
the one kept on the shadow stack or directly uses the one on the shadow stack.
Shadow stacks can be categorized into two types based on how the return address
on them is referred to: traditional~\cite{RAD:ICDCS01} or
parallel~\cite{SS:AsiaCCS15}. We summarize from two shadow stack
papers~\cite{SS:AsiaCCS15,SSSok:Oakland19} about these two classes of shadow 
stacks in the following subsections. 

%------------------------------------------------------------------------------%
\subsubsection{Traditional Shadow Stack}
\label{section:survey:shadow:css}
%------------------------------------------------------------------------------%

\begin{figure}[h]
    \centering
    \resizebox{\columnwidth}{!}{
        \includegraphics{figs/shadow_stack}
    }
    \caption{Traditional Shadow Stack (left) and Parallel Shadow Stack (right)}
    \label{fig:shadow_stack}
\end{figure}

The left figure in Figure~\ref{fig:shadow_stack} shows a typical traditional
shadow stack. It has a shadow stack pointer (SSP) that always points to the top
of the shadow stack, just like the regular stack pointer pointing to the top of
the regular stack. For each function call, right before the call or in the
prologue of the callee, the SSP and the shadow stack is updated to save the
return address. Symmetrically, after the callee finishes executing, in the
epilogue or right after the call instruction in the caller, the shadow stack
pops the return address to validate the integrity of the return address on the
regular stack. Or in the epilogue it simply uses the return address from the
shadow tack to return, ignoring the one on the regular stack.

There are two common ways of implementing the SSP. The simplest one is to
reserve a general-purpose register for it. On a 32-bit x86 system, there are
only 8 general-purpose registers; missing one register could highly increase the
register pressure and thus affect the performance badly. However, Burow et al.
shows that reserving one general-purpose register for SSP on a x64\_64 system 
has very low overhead as there are 16 of them~\cite{SSSok:Oakland19}. The other 
way is to define a global variable for SSP. Every time the SSP is needed to
save/pop a return address or to be updated, the global variable is
loaded/stored from/to the regular stack. This option could be slow because load
and store instructions are time-consuming compared to pure register operations.

A special case worth attention in the implementation of a traditional shadow
stack is when {\tt setjmp}/{\tt longjmp} happens, which can unwind more than one
stack frames at once. It breaks the one-on-one call-return assumption. One
solution is to keep popping the return address from the shadow stack until one
matches or the shadow stack is empty~\cite{RAD:ICDCS01}. Dang et al. mentioned
one scenario that complicates the situation even more: if a function is called
more than once before {\tt longjmp}, the solution just mentioned could
fail. This problem can be solved by storing the regular stack pointer along with
the return address onto the shadow stack~\cite{DISE:WASSA}.


%------------------------------------------------------------------------------%
\subsubsection{Parallel Shadow Stack}
\label{section:survey:shadow:pss}
%------------------------------------------------------------------------------%
%
% - how it works
% - benefits
% - drawback

The right figure in Figure~\ref{fig:shadow_stack} shows a typical parallel
shadow stack. It does not need to keep an explicit shadow stack pointer (SSP)
because it uses a constant offset from the regular stack pointer to refer to the
items on the shadow stack.  In the figure, the memory distance between the
location of function {\tt foo}'s return address on the regular stack and on the
shadow stack is the same as the one for function {\tt bar}. 

The benefit of this design is obvious: it saves one valuable register or all the
load\&store instructions to maintain the SSP. Therefore, it has very good
performance. Besides, because of the one-on-one match between the return
addresses on the regular and shadow stack, it naturally handles the {\tt
setjmp}/{\tt longjmp} problem. The major disadvantage of a parallel stack is
that it incurs high memory overhead: the shadow stack requires to be as large as
the regular stack, while a traditional shadow stack only needs to allocate space
for return addresses and possibly regular stack pointers that are live on the
regular stack. Burow et al. mentioned two more drawbacks of parallel shadow
stacks~\cite{SSSok:Oakland19}. We will discuss them in
Section~\ref{section:design:ss} and explain why these two problems should not be
severe concerns on {\ISA} systems.


==> tables/code_size.tex <==
%
% Code size overhead table.
%
\begin{table}[ptb]
\centering
\sffamily
\footnotesize{
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
& \textbf{Baseline} & {\bf SS} & {\bf SP} & {\bf CFI} & {\bf Silhoue-} & {\bf Invert} & {\bf SSFI} \\
& {\bf (\# bytes)} & {\bf (\%)} & {\bf (\%)} & {\bf (\%)} &{\bf tte (\%)} & {\bf (\%)} & {\bf (\%)} \\
\midrule
bubblesort & 1,424 & 4.92 & 181.46 & 1.26 & 46.91 & 8.15 & 53.37 \\
ctl-string & 1,422 & 6.05 & 19.41 & 1.27 & 26.72 & 9.56 & 43.32 \\
cubic & 1,984 & 3.53 & 17.14 & 0.91 & 21.57 & 5.85 & 23.89 \\
dijkstra & 1,656 & 4.83 & 31.16 & 1.09 & 37.08 & 7.85 & 75.00 \\
edn & 3,230 & 1.86 & 10.34 & 0.56 & 12.76 & 3.16 & 34.12 \\
fasta & 1,292 & 4.64 & 16.41 & 1.39 & 22.45 & 7.89 & 30.80 \\
fir & 854 & 7.03 & 18.27 & 2.11 & 27.40 & 11.94 & 36.30 \\
frac & 1,320 & 5.30 & 22.12 & 1.36 & 28.79 & 8.79 & 36.97 \\
huffbench & 4,980 & 1.20 & 22.13 & 0.36 & 23.69 & 2.05 & 45.22 \\
levenshtein & 2,116 & 3.31 & 23.53 & 0.85 & 27.69 & 5.48 & 42.82 \\
matmult-int & 2,030 & 3.45 & 14.48 & 0.89 & 18.82 & 5.71 & 35.86 \\
nbody & 3,418 & 1.76 & 15.27 & 0.53 & 17.55 & 2.98 & 17.96 \\
ndes & 4,306 & 1.86 & 19.65 & 0.42 & 21.92 & 3.02 & 32.19 \\
nettle-aes & 2,960 & 2.70 & 11.62 & 0.74 & 15.07 & 4.53 & 30.74 \\
picojpeg & 15,834 & 1.05 & 17.04 & 0.11 & 18.20 & 1.57 & 56.08 \\
qrduino & 17,276 & 0.52 & 15.54 & 0.10 & 16.16 & 0.83 & 33.16 \\
rijndael & 9,828 & 0.81 & 9.85 & 0.18 & 10.85 & 1.32 & 35.84 \\
sglib-dllist & 1,618 & 3.71 & 16.19 & 1.11 & 21.01 & 6.30 & 48.58 \\
sglib-listinsertsort & 930 & 6.45 & 17.42 & 1.94 & 25.81 & 10.97 & 38.28 \\
sglib-listsort & 1,320 & 4.55 & 15.76 & 1.36 & 21.67 & 7.73 & 49.39 \\
sglib-queue & 1,988 & 3.02 & 35.41 & 0.91 & 39.34 & 5.13 & 108.55 \\
sglib-rbtree & 1,614 & 6.07 & 21.81 & 2.48 & 30.36 & 10.53 & 56.75 \\
slre & 4,376 & 2.33 & 10.92 & 0.41 & 13.67 & 3.56 & 30.07 \\
sqrt & 920 & 6.52 & 20.87 & 1.96 & 29.35 & 11.09 & 26.74 \\
st & 5,272 & 1.14 & 9.56 & 0.34 & 11.04 & 1.93 & 14.98 \\
stb\_perlin & 1,414 & 4.95 & 20.79 & 1.27 & 27.02 & 8.20 & 20.93 \\
trio-sscanf & 5,436 & 3.64 & 19.32 & 8.46 & 31.42 & 12.91 & 51.62 \\
whetstone & 2,618 & 2.67 & 15.28 & 0.69 & 18.64 & 4.43 & 28.11 \\
wikisort & 10,612 & 1.87 & 19.75 & 0.55 & 22.16 & 2.83 & 58.84 \\
\midrule
{\bf min (\%)} & & 0.52 & 9.56 & 0.10 & 10.85 & 0.83 & 14.98 \\
{\bf max (\%)} & & 7.03 & 181.46 & 8.46 & 46.91 & 12.91 & 108.55 \\
{\bf geo. mean (\%)} & & 3.49 & 21.57 & 1.22 & 23.35 & 6.02 & 40.19 \\
\bottomrule
\end{tabular}
}}
\caption{Code Size Overhead on BEEBS Benchmarks.SS: Shadow Stack; SP: Store Promotion.}
\label{table:codesize}
\end{table}


==> tables/stores.tex <==
%
% Summarize the properties of various store instructions.
%

\begin{table*}[tb]
    \centering
    \sffamily
    \ra{1.3}
    \small{
      \begin{tabular}{@{}lcl@{}}
        \toprule
        {\bf Property} & \phantom{abc} & {\bf Description} \\
        \midrule
        source register && A general-purpose register or a floating-point 
        register that contains the value to store. \\
        base register && A general-purpose register that contains the base
        address of the target memory address. \\
        offset register && A general-purpose register added to base register to
        compute the target address. \\
        immediate && Ranges from -255 to 4095. It is added to the base register 
        to compute the target memory address.\\
        left shift && When offset register is present, it can be optionally
        shifted left by up to 3 bits before being added to the base reigster. \\
        write back && The base register can be optionally updated to the 
        computed target memory address. \\
        store multiple && Store multiple registers to consecutive memory
        locations.\\
        \bottomrule
    \end{tabular}}
    \caption{Properties of {\ISA} Store Instructions}
    \label{table:store}
\end{table*}


==> tables/tcb.tex <==
\begin{table}[tb]
  \centering
  \sffamily
  %\ra{1.3}
  \small{
\begin{tabular}{@{}llr@{}}
\toprule
\textbf{Component} & \textbf{Language} & \textbf{SLOC} \\
\midrule
Shadow Stack Transform Pass & C++ & 462 \\
Store Promotion Pass & C++ & 740 \\
CFI Pass & C++ & 222 \\
Privileged Code Scanner & Bourne Shell & 95 \\
\addlinespace
\textbf{Total}     & & 1,519 \\
\bottomrule
\end{tabular}}
\caption{{\System} Source Lines of Code (SLOC)}
\label{table:tcb}
\end{table}

